Data-integrated uncertainty quantification for the performance prediction of iced airfoils

Airfoil icing is a severe safety hazard in aviation and causes power losses on wind turbines. The precise shape of the ice formation is subject to large uncertainties, so uncertainty quantification (UQ) is needed for a reliable prediction of its effects. In this study, we aim to establish a reliable estimate of the effect of icing on airfoil performance through UQ. We use a series of experimentally measured wind tunnel ice shapes as input data. Principal component analysis is employed to construct a set of linearly uncorrelated geometric modes from the data, which serves as random input to the UQ simulation. For uncertainty propagation, non-intrusive polynomial chaos expansion (NIPC), multi-level Monte Carlo (MLMC) and multi-fidelity Monte Carlo control variate (MFMC) methods are employed and compared. As a baseline model, large eddy simulations (LES) are carried out using the discontinuous Galerkin flow solver FLEXI. UQ simulations are carried out with the in-house framework PoUnce. Its focus is on a high level of automation and efficiency considerations in a high performance computing environment. Due to the high number of samples, the simulation tool chain of the baseline model is completely automatized, including a new structured boundary layer grid generator for highly irregular domain shapes. The results show that forces on the airfoil vary considerably due to the uncertain ice shape. All three methods prove to be suited to predict mean and standard deviation. In the Monte Carlo techniques, the choice and performance of low-fidelity models is shown to be decisive for estimator variance reduction. The MFMC method performs best in this study. To our knowledge, there are no UQ studies of iced airfoils based on LES, let alone with advanced UQ methods such as MLMC or MFMC. The present study thus represents a leap in accuracy and level of detail for this application.

==> Makefile <==
LATEX=pdflatex
LATEXOPT=--shell-escape -synctex=1
NONSTOP=--interaction=nonstopmode

LATEXMK=latexmk
LATEXMKOPT=-pdf

MAIN=paper.tex

all: 
	touch paper.glo
	rubber --module glossaries --synctex --unsafe -f --pdf -s --warn=all paper
	rubber-info --check paper

%.pdf: %.tex 
	cd $(dir $<); rubber --synctex --unsafe -f --pdf -s --warn=all $(notdir $<)

run:
	nohup ~/.goodies/scripts/detach.py okular --unique paper.pdf\#src:$(LINE)$(FILE) &
	nohup okular --unique paper.pdf\#src:$(LINE)$(FILE) &

clean:
	rubber --clean paper.tex

veryclean: clean
	\rm paper.gls paper.glg paper.glo paper.ist paper.abg paper.abi paper.acn paper.acr paper.alg paper.syg paper.syi paper.slg; true
	\rm paper.bbl paper.cb paper.cb2 paper.mw paper.glsdefs paper.pgf-plot.gnuplot paper.pgf-plot.table paper.toc;true
	\find . -name "*.aux" -exec rm {} \;
	\find . -name "*.fls" -exec rm {} \;
	\find . -name "*.fdb_latexmk" -exec rm {} \;

PHONY: 
	run clean


==> packages.tex <==
\RequirePackage{etex}
\usepackage{etoolbox}  % insert new e-TEX commands (required for \AfterEndEnvironment)

\usepackage[ruled,vlined]{algorithm2e}
%-------------------------------------------------------------------------------
% LANGUAGE
%-------------------------------------------------------------------------------
\usepackage[english]{babel} % Sprache 
\usepackage[utf8]{inputenc} % Tippen von Umlauten

%-------------------------------------------------------------------------------
% TEXT AND MATH FONT
%-------------------------------------------------------------------------------
%\setkomafont{sectioning}{\normalfont\bfseries}
%\usepackage{cmbright}  % Schriftart
%\input{cmbrightfix}    % dicke kleine Buchstaben in Formeln reparieren
%\usepackage{cmcaps}  % font for thanks
%\usepackage{calligra}  % font for thanks

\usepackage{textgreek}


%-------------------------------------------------------------------------------
% IMAGES / GRAPHICS
%-------------------------------------------------------------------------------
\usepackage{graphicx}

%-------------------------------------------------------------------------------
% FLOAT CONTROL
%-------------------------------------------------------------------------------
%\usepackage[section]{placeins} # Alle figures,tabellen, etc. innerhalb der section anorden
%\usepackage{float}
%\usepackage{afterpage}

%-------------------------------------------------------------------------------
% PDF-Output
%------------------------------------------------------------------------------
\usepackage{xcolor}
%\definecolor{lnkcol}{rgb}{0.,0.,0.0} %black
%\usepackage[pdftex,pdfpagelabels=true,hypertexnames=false]{hyperref}
%\hypersetup{pdfborder={0 0 0},
            %bookmarksnumbered=true,
            %pdftitle = {\myauthor: \mytitle},
            %pdfsubject = {},
            %pdfauthor = {\myauthor},
            %pdfkeywords = {},
            %colorlinks=true,
            %citecolor=lnkcol,%
            %linkcolor=lnkcol,%
            %urlcolor=lnkcol }
%\usepackage[all]{hypcap}  % hyperlink soll oberhalb des Bilds anhalten


%-------------------------------------------------------------------------------
% EQUATIONS
%-------------------------------------------------------------------------------
\usepackage{amssymb}
\usepackage{amsmath}
%\usepackage{amsthm}
\usepackage{breqn}
\usepackage{mathtools}

%-------------------------------------------------------------------------------
% TABULAR
%-------------------------------------------------------------------------------
\usepackage{tabularx}
\usepackage{multirow}


%%-------------------------------------------------------------------------------
%% OTHER USEFUL PACKAGES
%%-------------------------------------------------------------------------------
\usepackage{changebar}
\usepackage{csquotes}  % Anfuehrungszeichen (wird von glossaries empfohlen)
\usepackage{xspace}    % Leerzeichen oder nicht nach Kommando einfuegen

%\usepackage[all]{nowidow} % Witwen und Waisen (Hurenkinder, Schusterjungen) vermeiden
%\frenchspacing % No big horizontal spaces between sentences

\usepackage{pifont}


%%-------------------------------------------------------------------------------
%% FROM SG 19
%%-------------------------------------------------------------------------------

\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
\usepgfplotslibrary{colorbrewer}
\usepgfplotslibrary{colormaps} 
\usepgfplotslibrary{fillbetween}


\usepackage{amscd}
\usepackage{bm}
\usepackage{textcomp}

\usepackage{enumitem}
\setlength{\parskip}{0cm plus0.0cm minus0.0cm}











